JIGGLE: An Active Sensing Framework for Boundary Parameters Estimation in Deformable Surgical Environments

Surgical automation can improve the accessibility and consistency of life saving procedures. Most surgeries require separating layers of tissue to access the surgical site, and suturing to reattach incisions. These tasks involve deformable manipulation to safely identify and alter tissue attachment (boundary) topology. Due to poor visual acuity and frequent occlusions, surgeons tend to carefully manipulate the tissue in ways that enable inference of the tissue's attachment points without causing unsafe tearing. In a similar fashion, we propose JIGGLE, a framework for estimation and interactive sensing of unknown boundary parameters in deformable surgical environments. This framework has two key components: (1) a probabilistic estimation to identify the current attachment points, achieved by integrating a differentiable soft-body simulator with an extended Kalman filter (EKF), and (2) an optimization-based active control pipeline that generates actions to maximize information gain of the tissue attachments, while simultaneously minimizing safety costs. The robustness of our estimation approach is demonstrated through experiments with real animal tissue, where we infer sutured attachment points using stereo endoscope observations. We also demonstrate the capabilities of our method in handling complex topological changes such as cutting and suturing.

==> short_abstract.tex <==
Surgical tasks often involve deforming tissue to sever (or create via suturing) attachment points. 
Due to poor visual acuity and frequent occlusions, surgeons tend to carefully manipulate the tissue in ways that enable inference of the tissue’s current attachment points without causing unsafe tearing. 
Inspired by this approach, we propose our Joint Interactive Guided Gaussian Likelihood Estimation (\algname) framework for interactive sensing and estimation of unknown attachment points in deformable surgical environments. 
This framework has two key components: 
(1) an probabilistic estimation of the current attachment points through the use of a differentiable soft-body simulator paired with an extended Kalman filter, and 
(2) an active sensing pipeline that selects actions that maximize the information gain on its belief of the tissue attachment points while minimizing safety costs.  
The robustness of the estimation component of our framework is demonstrated on real animal tissue, where we infer sutured attachment points using a stereo endoscope for observations. 
The full framework is demonstrated in simulation, showcasing its ability to generate complex pulling and folding maneuvers to achieve information gain without exerting excessive force, thereby minimizing the risk of unsafe tearing. 
We also showcase our framework with complex topological changes like cutting and suturing.







%%%%%%%%%%%%% bad ones below %%%%%%%%%%%%%%%
Surgical automation can improve the accessibility and consistency of life-saving procedures. 
The start of most surgeries requires separating layers of tissue to access the surgical site. 
This involves deformable manipulation to safely identify and sever tissue attachment points. 
On the other hand, suturing tasks involve identifying and attaching free regions. 
Surgeons adapt to poor visual acuity and frequent occlusions in surgical environments by carefully interacting with tissues to understand their attachment points. 
In a similar fashion, we propose JIGGLE, a framework for estimation and interactive sensing of unknown boundary parameters in deformable surgical environments.  
This framework efficiently estimates tissue attachment points by using a differentiable soft-body simulator paired with an extended Kalman filter (EKF). 
The robot leverages our probabilistic estimation to select actions that maximize the information gain of 
the tissue attachment points.
We demonstrate the robustness of our estimation on real animal tissue, where we use stereo endoscope observations to infer sutured attachment points. 
Our active sensing results execute complex maneuvers to achieve information gain while avoiding unsafe tearing. 
We also showcase our framework with complex topological changes like cutting and suturing

%%%%%%%%%%%%% bad ones below %%%%%%%%%%%%%%%

Surgical automation has the potential to revolutionize healthcare by improving the accessibility and consistency of life-saving procedures. 
The start of most surgeries requires the separation of fascia and other tissue layers to clear the field of view and access the surgical site. 
This involves deformable manipulation to identify tissue attachment points and safely sever those boundary connections. 
On the other hand, suturing tasks involve identifying free regions and creating attachments to bind them together. 
Surgeons adapt to poor visual acuity and frequent occlusions of attachments by interacting with and carefully tensioning tissues to understand their attachment points. 
In a similar fashion, we propose JIGGLE, a framework for estimation and interactive sensing of unknown boundary parameters in deformable surgical environments. 
% Poor visual acuity and frequent occlusions make inferring these attachments solely through observations infeasible, necessitating the need for active (yet safe) interaction. 
% In this work, we propose our Joint Interactive Guided Gaussian Likelihood Estimation (\algname) framework for interactive sensing and estimation of unknown attachment points in deformable surgical environments. 
Our framework efficiently estimates the current tissue attachment points by using a differentiable soft-body simulator paired with an extended Kalman filter (EKF). 
%The estimation component of the framework uses a differentiable soft-body simulator to construct an extended Kalman filter for efficient estimation and tracking of unknown boundary parameters in surgical environments. 
The robot leverages the probabilistic nature of this estimation to select actions that maximize the information gain of %its belief of 
the tissue attachment points.
The robustness of our estimation approach is demonstrated on real animal tissue, where we infer sutured attachment points using stereo endoscope observations. 
Our active sensing simulation results show the ability to generate complex 
% pulling and folding 
control
maneuvers to achieve information gain 
while avoiding unsafe tearing.
% thereby minimizing the risk of unsafe tearing. 
We also showcase our framework with complex topological changes like cutting and suturing.

%%%%%%%%%%%%%%% MORE ABSTRACTS %%%%%%%%%%%%%


JOINT ABOVE

BACKUP OF JOINT 
Surgical automation can improve the accessibility and consistency of life-saving procedures. 
The start of most surgeries requires separating layers of tissue to access the surgical site. 
This involves deformable manipulation to safely identify and sever tissue attachment points. 
On the other hand, suturing tasks involve identifying and attaching free regions. 
% Surgeons adapt to poor visual acuity and frequent occlusions in surgical environments by carefully interacting with tissues to understand their attachment points. 
Due to poor visual acuity and frequent occlusions, surgeons tend to carefully manipulate the tissue in ways that enable inference of the tissue’s  attachment points without causing unsafe tearing. 

In a similar fashion, we propose JIGGLE, a framework for estimation and interactive sensing of unknown boundary connectivity in deformable surgical environments. 
This framework has two key components: 
(1) a probabilistic estimation for the current attachment points, achieved by integrating a differentiable soft-body simulator with an extended Kalman filter (EKF), and
(2) an optimization-based active control pipeline that identifies actions to maximize information gain of the tissue attachment points,  
% regarding its belief in the tissue attachment points, 
while simultaneously minimizing safety costs.
The robustness of our estimation approach is demonstrated on data from real animal tissue, where we infer sutured attachment points using stereo endoscope observations. We also demonstrate the capabilities of our designed active sensing controller in handling complex topological changes such as cutting and suturing.


FEI DONT EDIT ABOVE

% Surgical tasks often involve deforming tissue to sever (or create via suturing) attachment points. 
% Due to poor visual acuity and frequent occlusions, surgeons tend to carefully manipulate the tissue in ways that enable inference of the tissue’s current attachment points without causing unsafe tearing. 
% Inspired by this approach, we propose our Joint Interactive Guided Gaussian Likelihood Estimation (\algname) framework for interactive sensing and estimation of unknown attachment points in deformable surgical environments. 
% This framework has two key components: 
% (1) an probabilistic estimation of the current attachment points through the use of a differentiable soft-body simulator paired with an extended Kalman filter, and 
% (2) an active sensing pipeline that selects actions that maximize the information gain on its belief of the tissue attachment points while minimizing safety costs.  
% The robustness of the estimation component of our framework is demonstrated on real animal tissue, where we infer sutured attachment points using a stereo endoscope for observations. 
% The full framework is demonstrated in simulation, showcasing its ability to generate complex pulling and folding maneuvers to achieve information gain without exerting excessive force, thereby minimizing the risk of unsafe tearing. 
% We also showcase our framework with complex topological changes like cutting and suturing.


% Surgical automation has the potential to revolutionize healthcare by improving the accessibility and consistency of life-saving procedures. 
% The start of most surgeries requires the separation of fascia and other tissue layers to clear the field of view and access the surgical site. 
% This involves deformable manipulation to identify tissue attachment points and safely sever those boundary connections. 
% On the other hand, suturing tasks involve identifying free regions and creating attachments to bind them together. 
% Surgeons adapt to poor visual acuity and frequent occlusions of attachments by interacting with and carefully tensioning tissues to understand their attachment points. 
Fei's version : 

Surgical tasks often involve deforming tissue to sever (or create via suturing) attachment points. 
Due to poor visual acuity and frequent occlusions, surgeons tend to carefully manipulate the tissue in ways that enable inference of the tissue’s current attachment points without causing unsafe tearing. 
In a similar fashion, we propose JIGGLE, a framework for estimation and interactive sensing of unknown boundary connectivity in deformable surgical environments. 
This framework has two key components: 
(1) a probabilistic estimation for the current attachment points, achieved by integrating a differentiable soft-body simulator with an extended Kalman filter (EKF), and
(2) an optimization-based active control pipeline that identifies actions to maximize information gain of the tissue attachment points,  
% regarding its belief in the tissue attachment points, 
while simultaneously minimizing safety costs.
The robustness of our estimation approach is demonstrated on data from real animal tissue, where we infer sutured attachment points using stereo endoscope observations. We also demonstrate the capabilities of our designed active sensing controller in handling complex topological changes such as cutting and suturing.
